Industrial Application of the Shapley value-based Redispatch Cost Allocation to Large-Scale Power Grids requires AC Optimal Power Flow

A burgeoning topic in the current energy transition are the huge costs of redispatch congestion management (CM) in large transmission systems. One of the German transmission system operators (TSOs) raised the critical inquiry of how to allocate the redispatch costs amongst TSOs in an equitable and beneficial way. Previously, a Shapley value-based approach has been introduced on small test grids, using the linear DC approximation of optimal power flow (OPF). However, within the application of CM, its feasibility and accuracy for large-scale power grids and its impact on the computed congestions remain uncertain. Therefore, this study investigates the applicability of the DC OPF compared to the exact AC OPF with regard to the Shapley values, for both small and large-scale grids. Numerical simulation shows significant differences in the congested lines, the overall redispatch costs, and the Shapley values. These findings suggest that for future CM, the TSOs should further investigate AC OPF solutions.

==> ACM_files_OLD/ACM_infos.tex <==
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

\acmYear{2024}\copyrightyear{2024}
\setcopyright{acmlicensed}
\acmConference[e-Energy '24]{The Fourteenth ACM International Conference on Future Energy Systems}{ June 4 - 7, 2024}{Virtual Event, USA}
\acmBooktitle{The Fourteenth ACM International Conference on Future Energy Systems (e-Energy '24),  June 4 - 7, 2024, Virtual Event, USA}
\acmPrice{}
\acmDOI{}
\acmISBN{}

==> sections/authors.tex <==
\authoranon{
\author{Rebecca Bauer}
\email{rebecca.bauer@kit.edu}
\affiliation{%
  \institution{Institute of Automation and Applied Informatics, Karlsruhe Institute of Technology}
    \country{Germany}
}
}

\authoranon{
\author{Xinliang Dai}
\email{xinliang.dai@kit.edu}
\affiliation{%
  \institution{Institute of Automation and Applied Informatics, Karlsruhe Institute of Technology}
    \country{Germany}
}
}

\authoranon{
\author{Veit Hagenmeyer}
\email{veit.hagenmeyer@kit.edu}
\affiliation{%
  \institution{Institute of Automation and Applied Informatics, Karlsruhe Institute of Technology} 
  \country{Germany}
}
}

\renewcommand{\shortauthors}{\textanon{Bauer et al.}}

==> sections/experimental_setup.tex <==
\section{Experimental Setup}

\subsection{Grids \& Modifications}
\begin{itemize}
    \item PGLib modifications
    \item describe table
    \item describe HV or EHV levels
\end{itemize}

\begin{table}[htbp!]
    \caption{Test cases. \textcolor{red}{add: total load/gen capacity / nr generators}} \label{TB::numerical-result}
    \centering
    \scriptsize
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{ccccccc}\toprule
        \multicolumn{4}{c}{} & \multicolumn{3}{c}{Runtime (OPF)} \\
        \cline{5-7}
        \multicolumn{1}{c}{Case} & \multicolumn{1}{c}{Busses} & \multicolumn{1}{c}{Lines} & \multicolumn{1}{c}{congestions} & \multicolumn{1}{c}{DC} & \multicolumn{1}{c}{AC} & \multicolumn{1}{c}{ALADIN} \\\hline
        case9 & 9 & 9 & 1 & & &  \\
        case39 & 39 & & & & & \\
        case300 & 300 & & & & & \\
        case793 & 793 & & & & & \\
        case1354wp & 1354 & & & & & \\
        case2383 & 2383 & & & & & \\
        \bottomrule
    \end{tabular}
\end{table}

% \subsubsection*{Research questions}
% \begin{itemize}
%     \item \textit{\textbf{Input requirements} - How does the input data / grid have to look?}
%     \item \textit{Scalability - how well does the algorithm perform on large networks?}
%     \begin{itemize}
%         \item Expectation: Largely depends on number of congestions, large networks are fine.
%     \end{itemize}
%     \item \textit{DC/AC - how much differ the results for AC OPF to DC OPF - is AC worth it?}
%     \begin{itemize}
%         \item Expectation: The results will differ quite a lot for large networks
%     \end{itemize}
%     \item \textit{How many partitions are useful for ALADIN?}
%     \begin{itemize}
%         \item Expectation: The fewer, the better - tradeoff with computation time
%     \end{itemize}
%     \item \textit{Parallel computing} - in MATLAB
% \end{itemize}

% \subsubsection*{Testing dimensions}
% \begin{itemize}
%     \item \textbf{Grid sizes:} 9, 39\_merged, 149 (BaWue), 300, 1354pegase, 2383wp, RTE, US
%     \begin{itemize}
%         \item take only networks that are reliable according to PGLib Report \cite{joszACPowerFlow2016}
%     \end{itemize}
%     \item \textbf{OPF:} DC/AC/distributed AC (ALADIN)
%     \item \textbf{Partitions:} few-many
% \end{itemize}
